Dichoptic Foveation

Interocular differences in visual perception can induce a variety of effects when fused by the brain. For example, prior works have found that carefully crafted binocular differences in local detail can improve contrast. It has also been found that when the frequency content of two stimuli are slightly different, blur suppression leads to a fused percept that is typically dominated by the sharper image. In this paper, we develop a psychophysical framework to measure the perception of natural image stimuli with interocular frequency differences across the visual field. To this end, we study the effect of dichoptic foveation, which we define as the application of blur to one eye and a simultaneous sharpening filter to the other. Stimuli were viewed in a virtual reality (VR) head-mounted display (HMD) and placed at different retinal eccentricities. Study data were scaled to a perceptual just objectionable difference (JOD) scale, and a 4D model was fit to it; our results suggest that interocular frequency differences can be well described by a simple computational model. We applied the model in a realistic VR scenario with free exploration of 360{\deg} videos to improve a base foveated rendering system by enhancing high frequency information dichoptically.

==> conf/packages.tex <==
%%% Language %%%%
% \RequirePackage[english]{babel}                  % Hyphenation and date format
\RequirePackage{xspace}                          % Abbreviation spacing
% \RequirePackage{xpunctuate}                      % Abbreviation spacing

%%% Tex-scripting %%%
\RequirePackage{ifthen}                          % If-then-else latex logic
% \RequirePackage{soul}                            % Underlining and Strike-through
% \RequirePackage{xargs}                           % For \newcommandx

%%% Color %%%
\RequirePackage{color}                           % Draft annotation coloring

%%% Math-mode %%%
\RequirePackage{amsmath}                         % Math equations
\RequirePackage{bm}                              % Math bold symbols

%%% Cross-referencing %%%
% \RequirePackage[toc,page,titletoc]{appendix}     % Appendix section
\RequirePackage[toc,titletoc]{appendix}  
\RequirePackage[capitalize,nameinlink]{cleveref} % Easy to use cross-referencing
\crefname{supp}{Supplement}{Supplements}     % Supplement section name setting

%%% Figures %%%
\RequirePackage{caption}                         % Figure captions
\RequirePackage{subfig}                          % Nested figures
% \usepackage[table]{xcolor}

\usepackage{enumitem}
